Efficient Multitask Learning on Resource-Constrained Systems

We present Antler, which exploits the affinity between all pairs of tasks in a multitask inference system to construct a compact graph representation of the task set and finds an optimal order of execution of the tasks such that the end-to-end time and energy cost of inference is reduced while the accuracy remains similar to the state-of-the-art. The design of Antler is based on two observations: first, tasks running on the same platform shows affinity, which is leveraged to find a compact graph representation of the tasks that helps avoid unnecessary computations of overlapping subtasks in the task set; and second, tasks that run on the same system may have dependencies, which is leveraged to find an optimal ordering of the tasks that helps avoid unnecessary computations of the dependent tasks or the remaining portion of a task. We implement two systems: a 16-bit TI MSP430FR5994-based custom-designed ultra-low-power system, and a 32-bit ARM Cortex M4/M7-based off-the-shelf STM32H747 board. We conduct both dataset-driven experiments as well as real-world deployments with these systems. We observe that Antler's execution time and energy consumption are the lowest compared to all baseline systems and by leveraging the similarity of tasks and by reusing the intermediate results from previous task, Antler reduces the inference time by 2.3X -- 4.6X and saves 56\% -- 78\% energy, when compared to the state-of-the-art.

==> tex/02_background.tex <==
\newpage
\section{Background and Motivation}
\label{sec:background}

\subsection{Multitask Learning}

Multitask learning refers to a genre of machine learning algorithms that jointly train two or more learners to increase their accuracy as well as their ability to generalize well by sharing the common knowledge in them~\cite{caruana1997multitask, ruder2017overview,zhang2017overview,zhang2017survey}. A wide variety of multitask learning approaches have been proposed in the literature which includes common feature learning~\cite{liu2017adversarial,zhang2016deep,misra2016cross,liu2015multi,mrkvsic2015multi,li2014heterogeneous,zhang2014facial}, task clustering~\cite{zhou2015flexible,barzilai2015convex,han2015learning,kumar2012learning,kang2011learning,thrun1996discovering}, task relation learning~\cite{long2017learning,lee2016asymmetric,zhang2013learning,zhang2013multilabel}, and low-rank optimization~\cite{yang2016trace,han2016multi,mcdonald2014spectral,agarwal2010learning,chen2009convex,zhang2008flexible}. 

The key technique behind all multitask learning methods is to share a subset of parameters among the learners, e.g., weights of the first few layers of the network networks, to enable sharing of learned representations of related tasks. This process improves the accuracy and generalization ability of each learner because most learning tasks can be broken down into multiple sequential stages and early stages of many tasks are often similar and sometimes the same. An analogy from biological learning would be how a human child first learns to recognize faces and then uses that knowledge to learn new tasks such as object recognition.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[height=1in]{figure/placeholder.PNG}
%     \caption{Multitask learning via hard parameter sharing.}
%     \label{fig:mtlbg}
%     %\vspace{-20pt}
% \end{figure}

\subsection{System Considerations}

The primary objective of multitask learning is to increase the accuracy and robustness of classifiers via knowledge sharing. This is implemented by introducing constraints on parameters across multiple learners during the joint training phase. Like any neural network training algorithm, however, this too has randomness built into it, e.g., parameter initialization and dropout, and as a consequence, the resultant networks are not unique, and the parameters that are shared among networks are not always the same ones. In other words, the same level of inference accuracy is achievable by a set of learners while sharing their network parameters in many different ways. Although this is not an issue in the mainstream multitask learning literature which is primarily concerned with inference accuracy, from a systems perspective, the time and energy cost of executing these \emph{similarly-accurate but architecturally-different} multitask learners are not the same.   

%How embedded DNN gets stored and executed
%Embedded System memory and CPU ideas and table
%Overheads/measurements of vanilla: inference time and energy, what percent is IO

The time and energy cost of performing neural network inference on an embedded system depends on both the amount of CPU-bound operations, which are largely a series of matrix multiplication and accumulation operations, as well as on the frequency of I/O operations to load the neural network parameters such as the weights into the main memory (i.e., RAM) from the non-volatile storage, e.g., EEPROM, flash, or FRAM. In certain learning scenarios, e.g., online~\cite{hoi2021online}, reinforcement~\cite{kaelbling1996reinforcement}, and federated learning~\cite{lim2020federated}, the network weights are often updated at runtime and need to be written back to non-volatile storage, which incurs additional overhead. 

In high-end machines that have powerful CPUs and large RAMs, I/O overheads as such is negligible. However, for low-resource, battery-powered IoT devices, the I/O overhead of frequent swapping in and out of classifiers between the main memory and the non-volatile storage is significant for two main reasons. First, the size of the internal RAM on these systems ranges from a few KB to a few hundred KB. The size of a neural network, on the other hand, is generally larger than this. Therefore, the CPU has to read in the network weights from flash at a frequency that is proportional to the ratio of the internal RAM and the size of the neural network. Second, multitask learning amplifies this overhead even more as it requires the system to execute more than one neural network. Recently, there have been multiple proposals~\cite{nwv, yono} to 
squeeze multiple neural networks to a size as small as 256KB to fit them in the main memory of an MCU, these methods do not guarantee inference accuracy as the number of neural networks increases.     

%studies have shown that a neural network compressed down to a few hundred KB ($10^6$ parameters) yields reasonably accurate inference results when the number of output classes is limited.            
 
\begin{figure}[!htb] 
    \centering
    \subfloat[]
    {
        \includegraphics[width = 0.223\textwidth]{figure/io_time_overhead.pdf}
    }
    \subfloat[] 
    {
        \includegraphics[width = 0.22\textwidth]{figure/io_energy_overhead.pdf}
    }
    \caption{Time and energy cost of multitask inference.} 
    \vspace{-15pt}
    \label{fig:iopercent} 
\end{figure} 


% \begin{table}[!htb]
%     \centering
%     \begin{tabular}{|l|l|l|}
%         \hline
%         \textbf{CPU}     & \textbf{16-bit}    & \textbf{32-bit} \\
%         \hline
%         Time    & 5 sec     & 1 sec \\
%                 & 25\% overhead & 5\% overhead \\
%         \hline        
%         Energy  & 100 mJ     & 5J \\
%                 & 10\% overhead & 30\% overhead \\
%             \hline
%     \end{tabular}
%     \caption{Time and energy overheads of multitask inference.}
%     \label{tab:iopercent}
% \end{table}

To demonstrate the time and energy cost of executing multiple neural networks on a low-resource system, we conduct an experiment where we execute three pre-trained neural networks of sizes 35KB, 100KB, and 132KB on a 16-bit MSP430 MCU as well as on a 32-bit Raspberry Pi Pico (PR2040). The networks are stored in the FRAM and the flash of these two systems, respectively, and they are executed sequentially. We measure the inference time and energy to process one input sample through all networks and break it down into in-memory inference and weight-reloading overhead. In Figure~\ref{fig:iopercent}, we observe that 16-bit MSP430 takes up to 6X more time per inference than 32-bit RP2040, but consumes $20\%-60\%$ less energy. Overall, we observe a $6\%-15\%$ time overhead and $8\%-24\%$ energy overhead --- which is significant in a low-resource system.    

From the experiment above, it is evident that a faster CPU cannot solve the overhead problem entirely. It reduces the inference time at the cost of a higher energy overhead and thus significantly reduces the battery life. One could argue that by choosing a low-power system that comes with a larger RAM could mitigate the problem. But in practice, chip manufacturers do not offer large RAMs in 16-bit MCUs due to cost, size, and overheating concerns. Later in this paper, we propose a new platform that uses multiple external FRAM chips as an energy-efficient and relatively faster alternative to flash memory. But that too has its time and energy overheads. In short, the time and energy overhead in multitask learning on low-resource systems cannot be solved using hardware provisioning only. We need intelligent algorithms in combination with better hardware design to address this issue.        

%\note{prove this overhead isicant.}  
%Argument - Does more memory or more CPU solve the problem?  
 


==> tex/08_discussion.tex <==
\section{Discussion}

\parlabel{Fine-Grained Task Decomposition.}
Although \sys uses only three branch points to in our experiments, it can be easily extended to have more fine-grained decomposition to form more compact task graphs. Such fine-grained decomposition of tasks might be necessary when the number of tasks is above 20. 

\parlabel{Optimization Alternatives.} \sys's task graph formation and task ordering are formed as two independent optimization problems and solved independently. We choose this design to make task ordering flexible so that dynamic constraints can be handled flexibly. An alternative approach such as joint optimization of task graph formation and execution order determination is possible but the downside is that if task dependencies change, the optimization problem has to be solved again.           

\parlabel{Generalization to Other Systems.} Although \sys is motivated by the constraints of a low-resource system, some of the techniques such as affinity-aware task graphs that execute under constraints and optimal ordering of tasks should apply to server-grade larger multitask inference systems as well. Cloud-based inference systems that execute more complex and larger number of inference tasks, exploiting task affinity could help reduce a server's response time.

\parlabel{Generalization to Other Workloads.} Although \sys's scope is limited to neural networks, the concept of tasks, task affinity, and task graphs are generalizable to any workload where a task can be factored into subtasks, compared, and merged. \sys is readily applicable to many non-neural classifiers such as decision tree and random forest that process data in stages.        

\parlabel{Improvement Over \sys.} \sys's advantage over the state-of-the-art in-memory multitask learning systems~\cite{nwv, yono} is its ability to reduce time and energy cost while offering the same level of accuracy. \sys, however, consumes more memory than these systems. We envision that \sys will inspire new techniques that will not only reduce time and energy overhead of multitask inference on embedded systems but also improve inference accuracy and perform complete in-memory execution of tasks.  

%These devices will be self-contained, long lasting, and feature-packed with several on-device classifiers. 


